Online Learning Using Only Peer Prediction

This paper considers a variant of the classical online learning problem with expert predictions. Our model's differences and challenges are due to lacking any direct feedback on the loss each expert incurs at each time step $t$. We propose an approach that uses peer prediction and identify conditions where it succeeds. Our techniques revolve around a carefully designed peer score function $s()$ that scores experts' predictions based on the peer consensus. We show a sufficient condition, that we call \emph{peer calibration}, under which standard online learning algorithms using loss feedback computed by the carefully crafted $s()$ have bounded regret with respect to the unrevealed ground truth values. We then demonstrate how suitable $s()$ functions can be derived for different assumptions and models.

==> proof_main.tex <==
\subsection*{Proof of Theorem \ref{main:convergence}}

\begin{proof}
We list the key steps in the proof. 

\noindent \textbf{Step 1} Using Martingale inequality we know
\begin{align*}
&\sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{p_t,t}  \rightarrow \sum_{t=1}^T g(p_a(t),p_t),\\
&\sum_{t=1}^T \ell_{a(t),t} - \sum_{t=1}^T \ell_{p_t,t}  \rightarrow \sum_{t=1}^T f(p_a(t),p_t)
\end{align*}
In particular, from Eqn. (\ref{conv:S}), with probability at least $1-2\delta$, 
the following holds:
\begin{small}
\begin{align*}  %\label{e:genT}
\biggl |\sum_{t=1}^T s_{a(t),t}& - \sum_{t=1}^T s_{p_t,t}  \\
&- \sum_{t=1}^T g(p_a(t),p_t)\biggr |  \leq \Et_{mart}(\delta, \sigma_g, T)\\
\biggl |\sum_{t=1}^T s_{a^*_{peer},t}& - \sum_{t=1}^T s_{p_t,t} \\
&- \sum_{t=1}^T g(p_{a^*_{peer}}(t),p_t)\biggr | \leq \Et_{mart}(\delta, \sigma_g, T)
\end{align*}
\end{small}
Similarly with probability at least $1-2\delta$,  
\begin{small}
\begin{align*} % \label{e:genT}
\biggl |\sum_{t=1}^T \ell_{a(t),t} &- \sum_{t=1}^T \ell_{p_t,t}\\
&  - \sum_{t=1}^T f(p_a(t),p_t)\biggr |  \leq \Et_{mart}(\delta, 2, T)\\
\biggl |\sum_{t=1}^T \ell_{a^*_{peer},t}& - \sum_{t=1}^T \ell_{p_t,t} \\
&- \sum_{t=1}^T f(p_{a^*_{peer}}(t),p_t)\biggr | \leq \Et_{mart}(\delta, 2, T)
\end{align*}
\end{small}




\paragraph{Step 2} Via Lemma \ref{cali:g}, we know with probability at least $1-\delta_g$ that $a^*_g = a^*_{peer}$. Using facts in Step 1, we know the following holds with probability at least $1-\delta_g$:
\begin{align*}
&\sum_{t=1}^T g(p_a(t),p_t)-\sum_{t=1}^T g(p_{a^*_g}(t),p_t) \\
\leq &\sum_{t=1}^T g(p_a(t),p_t)-\sum_{t=1}^T s_{a(t),t} + \sum_{t=1}^T s_{p_t,t}  \\
+ & \sum_{t=1}^T s_{a^*_{g},t}-\sum_{t=1}^T s_{p_t,t}  -\sum_{t=1}^T g(p_{a^*_g}(t),p_t) \\
&~~+  \sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{a^*_{peer},t}\\
\leq & 2\Et_{mart}(\delta, \sigma_g, T) +\sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{a^*_{peer},t}% \Et_{online}(T,N) 
\end{align*}
The first inequality is because $\sum_{t=1}^T s_{a^*_{peer},t} \leq  \sum_{t=1}^T s_{a^*_g,t}$ (optimality of $a^*_{peer}$).



\paragraph{Step 3} By Proposition \ref{sum:calibrate} we know  \begin{small}
\begin{align*}
& \sum_{t=1}^T f(p_a(t),p_t) - \sum_{t=1}^T f(p_{a^*_f}(t),p_t) \\
\leq & T \cdot \psi^{-1} \biggl( \frac{\sum_{t=1}^T g(p_a(t),p_t) - \sum_{t=1}^T g(p_{a^*_g}(t),p_t)}{T}\biggr)\\
\leq & T \cdot \psi^{-1} \biggl (\frac{2\Et_{mart}(\delta, \sigma_g, T) + \sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{a^*_{peer},t}}{T}\biggr )
\end{align*}
\end{small}

\paragraph{Step 4} Then  
\begin{small}
\begin{align*}
 &\sum_{t=1}^T \ell_{a(t),t} - \sum_{t=1}^T \ell_{a^*,t} \\
 =&(\sum_{t=1}^T \ell_{a(t),t} - \sum_{t=1}^T \ell_{p_t,t}) - (\sum_{t=1}^T \ell_{a^*,t} - \sum_{t=1}^T \ell_{p_t,t})\\
 \leq & \sum_{t=1}^T f(p_a(t),p_t) - \sum_{t=1}^T f(p_{a^*}(t),p_t) + 2\Et_{mart}(\delta, 2, T) \\
 \leq & \sum_{t=1}^T f(p_a(t),p_t) - \sum_{t=1}^T f(p_{a^*_f}(t),p_t)+ 2\Et_{mart}(\delta, 2, T) \\
 \leq & T \cdot \psi^{-1} \biggl (\frac{2\Et_{mart}(\delta, \sigma_g, T) + \sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{a^*_{peer},t} }{T}\biggr )\\
 &~~~~ +2\Et_{mart}(\delta, 2, T)
\end{align*}
\end{small}

\paragraph{Step 5} From the guarantee of running an online learning algorithm, we have
\begin{align}
\EE\left[\sum_{t=1}^T s_{a(t),t}\right]-\sum_{t=1}^T s_{a^*_{peer},t} \leq \Et_{online}(T,N) 
\end{align}
Further 
\begin{small}
\begin{align*}
 &\EE\left[\sum_{t=1}^T \ell_{a(t),t}\right] - \sum_{t=1}^T \ell_{a^*,t} \\
 \leq & T \cdot \EE\left[ \psi^{-1} \biggl (\frac{2\Et_{mart}(\delta, \sigma_g, T) + \sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{a^*_{peer},t} }{T}\biggr )\right]\\
 &~~~~ +2\Et_{mart}(\delta, 2, T)\\
 \leq & T \cdot  \psi^{-1} \biggl (\frac{2\Et_{mart}(\delta, \sigma_g, T) +\EE\left[ \sum_{t=1}^T s_{a(t),t} - \sum_{t=1}^T s_{a^*_{peer},t}\right] }{T}\biggr )\\
 &~~~~ +2\Et_{mart}(\delta, 2, T)\quad \quad\quad\quad \text{(Concavity of $\psi^{-1}(\cdot)$)}\\
  \leq & T \cdot  \psi^{-1} \biggl (\frac{2\Et_{mart}(\delta, \sigma_g, T) +\Et_{online}(T,N)  }{T}\biggr )\\
 &~~~~ +2\Et_{mart}(\delta, 2, T).
 \end{align*}
 This completes the proof.
\end{small}
\end{proof}




